Data-Driven Output Regulation using Single-Gain Tuning Regulators

Current approaches to data-driven control are geared towards optimal performance, and often integrate aspects of machine learning and large-scale convex optimization, leading to complex implementations. In many applications, it may be preferable to sacrifice performance to obtain significantly simpler controller designs. We focus here on the problem of output regulation for linear systems, and revisit the so-called tuning regulator of E. J. Davison as a minimal-order data-driven design for tracking and disturbance rejection. Our proposed modification of the tuning regulator relies only on samples of the open-loop plant frequency response for design, is tuned online by adjusting a single scalar gain, and comes with a guaranteed margin of stability; this provides a faithful extension of tuning procedures for SISO integral controllers to MIMO systems with mixed constant and harmonic disturbances. The results are illustrated via application to a four-tank water control process.

==> Single Gain Tuning Regulator CDC/paperdefs.tex <==
\let\labelindent\relax
\let\proof\relax    % otherwise amsthm will error on \proof
\let\endproof\relax

% -------- Packages ---------
\usepackage{etex}
\usepackage[dvipsnames]{xcolor}
% \usepackage{pgfpages}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{mathrsfs}
\usepackage{siunitx}
\usepackage{verbatim}   % verbatim and comment environemtns		
\usepackage{mathtools}	% used for xmapsto command
\usepackage{siunitx}	% load SI units
\usepackage{mdframed}
\usepackage{graphicx}

% \usepackage[font=small]{caption}
% \usepackage{subcaption}
\usepackage[activate={true,nocompatibility},final,tracking=true,kerning=true,spacing=true,factor=1100,stretch=10,shrink=10]{microtype}
\usepackage[colorlinks,hidelinks]{hyperref}

\usepackage[style=ieee, backend=biber]{biblatex}
\renewcommand*{\bibfont}{\normalfont\footnotesize}

\usepackage{array}
\usepackage{multirow}
\usepackage{enumerate}
\usepackage{booktabs}

\usepackage{enumitem}
\usepackage{cuted}
\usepackage{arydshln}

% ----

\graphicspath{{./fig/}}



% %-------------------------------
% %-------- PGF-Plots ------------
% %-------------------------------

% \newcommand*{\strongconvex}{2}
% \newcommand*{\feedforward}{0.9}


% %http://pgfplots.sourceforge.net/gallery.html

% \usepackage{pgfplots}
% \pgfplotsset{width=8cm,compat=newest}
% \newcommand*{\damping}{0.006}%
% \newcommand*{\freq}{25}%
% \pgfmathsetmacro{\freqd}{sqrt(1-(\damping)^2)*\freq}%

% \pgfplotsset{
%     standard/.style={
%     axis x line=middle,
%     axis y line=middle,
%     enlarge x limits=0.15,
% 	enlarge y limits=0.15,
% 	%every axis x label/.style={at={(current axis.right of origin)},anchor=north west},
% 	%every axis y label/.style={at={(current axis.above origin)},anchor=north east},
% 	%x label/.style={at={(axis description cs:1.05,0.16)},anchor=north},
% 	%y label/.style={at={(axis description cs:0.2,1.05)},anchor=north},
% 	every axis plot post/.style={mark options={fill=black}},
% 	%every axis x label/.style={at={(current axis.right of origin)},anchor=north west},
%     %every axis y label/.style={at={(current axis.above origin)},anchor=north east}
% 	}
% }

% \pgfplotsset{%
%     ,compat=1.12
%     ,every axis x label/.style={at={(current axis.right of origin)},anchor=north west}
%     ,every axis y label/.style={at={(current axis.above origin)},anchor=north east}
%     }



%-------------------------
%--------- Tikz ----------
%-------------------------

\usepackage{tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.markings}
% \usetikzlibrary{snakes}
\usetikzlibrary{matrix}
\usetikzlibrary{calc}
\usetikzlibrary{patterns}
\usetikzlibrary{positioning}
\usetikzlibrary{shapes}
\usetikzlibrary{shapes.symbols}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{shadows.blur}
\usetikzlibrary{shapes.arrows}
\usetikzlibrary{shapes.multipart}
\usetikzlibrary{shapes.callouts}
\usetikzlibrary{shapes.misc}

\tikzstyle{every node}=[font=\small]
\tikzstyle{every path}=[line width=0.8pt,line cap=round,line join=round]
\newcommand{\midarrow}{\tikz \draw[-triangle 90] (0,0) -- +(.1,0);}


% %------- Circuit Tikz ----------
% \usepackage[american,smartlabels]{circuitikz}
% \ctikzset{bipoles/thickness=1}
% \ctikzset{bipoles/length=0.8cm}
% \ctikzset{bipoles/diode/height=.375}
% \ctikzset{bipoles/diode/width=.3}
% \ctikzset{tripoles/thyristor/height=.8}
% \ctikzset{tripoles/thyristor/width=1}
% \ctikzset{bipoles/vsourceam/height/.initial=.7}
% \ctikzset{bipoles/vsourceam/width/.initial=.7}


%------ My commands ---------
\DeclareMathAlphabet{\mathbbold}{U}{bbold}{m}{n}
\newcommand{\one}{\mathbbold{1}}
\newcommand{\zero}{\mathbbold{0}}

\newcommand{\real}{\mathbb{R}}
\newcommand{\mymod}[1]{\textup{mod}#1}
\newcommand{\realnonnegative}{\mathbb{R}_{\geq0}}
\newcommand{\until}[1]{\{1,\dots, #1\}}												
\newcommand{\complex}{\mathbb{C}}
\newcommand{\integer}{\mathbb{Z}}
\newcommand{\disk}{\mathbb{D}}
\newcommand{\mycircle}{\ensuremath{\mathbb S^{1}}}
\newcommand{\sphere}{\ensuremath{\mathbb S}}
\newcommand{\torus}{\ensuremath{\mathbb T}}
\newcommand{\setdef}[2]{\{#1 \;|\; #2\}}
\newcommand{\bigsetdef}[2]{\big\{#1 \; | \; #2\big\}}
\newcommand{\union}{\operatorname{\cup}}
\newcommand{\intersection}{\ensuremath{\operatorname{\cap}}}
\newcommand{\arc}{\textup{Arc}_{n}}
\newcommand{\bararc}{\overline{\mbox{Arc}}_{n}}
\newcommand{\PQ}{\textsf{PQ} }
\newcommand{\PV}{\textsf{PV} }
\newcommand{\mytt}[1]{\textup{\texttt{#1}}\xspace}
\renewcommand{\j}{\boldsymbol{\mathrm{j}}}
\renewcommand{\arc}{\operatorname{Arc}_{n}}
\newcommand{\abs}[1]{\left\lvert{#1}\right\rvert}                     			% \abs{x} -->  |x| with proper spacing
\DeclareMathOperator*{\minimize}{minimize} 									% minimize
\DeclareMathOperator{\subto}{subject~to}
\DeclareMathOperator{\proj}{Proj}
\DeclareMathOperator*{\maximize}{maximize} 									% maximize
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\sinc}{sinc}
\DeclareMathOperator*{\sinbf}{\mathrm{\bf sin}} 	                              %
\DeclareMathOperator*{\cosbf}{\mathrm{\bf cos}} 	                              %
\DeclareMathOperator*{\sincbf}{\mathrm{\bf sinc}} 	                              %

\DeclareMathOperator*{\arcsinbf}{\mathrm{\bf arcsin}} 	
\newcommand{\bsin}{\boldsymbol{\sin}}
\newcommand{\barcsin}{\boldsymbol{\arcsin}}
\newcommand{\bcos}{\boldsymbol{\cos}}
\newcommand{\bln}{\boldsymbol{\mathrm{ln}}}
                              

\newcommand{\vect}[1]{\mathbbold{#1}}
\newcommand{\vones}[1][]{\vect{1}_{#1}}
\newcommand{\vzeros}[1][]{\vect{0}_{#1}}
\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
\DeclareSymbolFontAlphabet{\mathbbold}{bbold}

\newcommand{\map}[3]{#1: #2 \rightarrow #3}
\newcommand{\setmap}[3]{#1: #2 \rightrightarrows #3}

\renewcommand{\Re}{\mathrm{Re}}
\renewcommand{\Im}{\mathrm{Im}}
\renewcommand{\deg}{\mathrm{deg}}

\renewcommand{\theenumi}{(\roman{enumi})}
\renewcommand{\labelenumi}{\theenumi}
%\renewcommand{\thefootnote}{\fnsymbol{footnote}}

\newcommand{\tr}{\color{red}}
\newcommand{\tv}{\color{violet}}
\newcommand{\tb}{\color{blue}}
\newcommand{\tg}[0]{\color{ForestGreen}}
\newcommand{\john}[1]{{\leavevmode\color{blue}\textbf{From John:\;}#1}}
\newcommand{\johnref}{\textbf{\textcolor{red}{[ref] }}}
\newcommand\fyimargin[1]{\marginpar{\color{violet} \small\ttfamily FYI (read and erase): #1}}
\newcommand{\todo}[1]{\par\noindent{\color{blue}\raggedright\textsc{#1}\par\marginpar{\large$\star$}}}
\newcommand{\fdmargin}[1]{\marginpar{\color{blue}\tiny\ttfamily{FD:} #1}}
\newcommand{\jsmargin}[1]{\marginpar{\color{red}\tiny\ttfamily{JS:} #1}}
\newcommand{\fbmargin}[1]{\marginpar{\color{red}\small\ttfamily{FB:} #1}}
\newcommand{\bpmargin}[1]{\marginpar{\bf \color{violet}\tiny\ttfamily{BP:} #1}}
\newcommand{\nmargin}[1]{\marginpar{\color{blue}\tiny\ttfamily{NM:} #1}}


% custom made commands
\newcommand*\fvec[1]{\ensuremath{\mathbf{#1}}}                           % creates a bold symbol
\newcommand{\transpose}{\mathsf{T}} %or \top or \intercal				% transpose symbol
\newcommand{\T}{\mathsf{T}} %or \top or \intercal				% transpose symbol


% Procend
\newcommand\oprocendsymbol{\hbox{$\square$}}
\newcommand\oprocend{\relax\ifmmode\else\unskip\hfill\fi\oprocendsymbol}
\def\eqoprocend{\tag*{$\square$}}

%Theorem Environments

% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{proposition}[theorem]{Proposition}
% % \newtheorem{proposition}{Proposition}[section]
% \newtheorem{problem}[theorem]{Problem}
% \newtheorem{remark}[theorem]{Remark}
% \newtheorem{assumption}[theorem]{Assumption}
% \newtheorem{example}[theorem]{Example}

%% nothing in the [] removes the roman numeral numbering; originally [section]
\newtheorem{theorem}{Theorem}[]
\newtheorem{lemma}{Lemma}[]
\newtheorem{corollary}{Corollary}[]
\newtheorem{proposition}{Proposition}

\theoremstyle{definition}
\newtheorem{definition}{Definition}[]
\newtheorem{assumption}{Assumption}[]
\newtheorem{problem}{Problem}[]

\theoremstyle{remark}
\newtheorem{remark}{Remark}[]
\newtheorem{example}{Example}[]


\newenvironment{pfof}[1]{\vspace{1ex}\noindent{\itshape Proof of #1:}\hspace{0.25em}} {\hfill\oprocend\vspace{1ex}}
\renewenvironment{proof} {\noindent{\itshape Proof:}\hspace{0.25em}} {\hfill\oprocend\vspace{1ex}}


% -------------------------------------
% ---------- Boyd Commands ------------
% -------------------------------------


\newcommand{\U}{\mathcal{U}}
\renewcommand{\P}{\mathcal{P}}


\newcommand{\ones}{\mathbf 1}
\newcommand{\reals}{{\mbox{\bf R}}}
\newcommand{\integers}{{\mbox{\bf Z}}}
\newcommand{\symm}{{\mbox{\bf S}}}  % symmetric matrices

\renewcommand{\ker}{\mathop{\rm ker}}
\renewcommand{\dim}{\mathop{\rm dim}}


\newcommand{\nullspace}{{\mathcal N}}
\newcommand{\range}{{\mathcal R}}
\newcommand{\Rank}{\mathop{\bf Rank}}
\newcommand{\Tr}{\mathop{\bf Tr}}
\newcommand{\diag}{\mathop{\bf diag}}
\newcommand{\card}{\mathop{\bf card}}
\newcommand{\rank}{\mathop{\bf rank}}
\newcommand{\conv}{\mathop{\bf conv}}

\newcommand{\Expect}{\mathop{\bf E{}}}
\newcommand{\Prob}{\mathop{\bf Prob}}
\newcommand{\Co}{{\mathop {\bf Co}}} % convex hull
\newcommand{\dist}{\mathop{\bf dist{}}}
\newcommand{\epi}{\mathop{\bf epi}} % epigraph
\newcommand{\Vol}{\mathop{\bf vol}}
\newcommand{\dom}{\mathop{\bf dom}} % domain
\newcommand{\intr}{\mathop{\bf int}}
\newcommand{\sign}{\mathop{\bf sign}}

\newcommand{\cf}{{\it cf.}}
\newcommand{\eg}{{\it e.g.}}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\etc}{{\it etc.}}



%---------- Signal Spaces ------------

%--------------------------------------------
%-------Norms and Inner Products-------------
%--------------------------------------------

\newcommand{\norm}[2]{\ensuremath{\|#1\|_{#2}}}
\newcommand{\bignorm}[1]{\ensuremath{\big \| #1 \big \|}}
\newcommand{\Bignorm}[1]{\ensuremath{\Big \| #1 \Big \|}}
\newcommand{\Biggnorm}[1]{\ensuremath{\Bigg \| #1 \Bigg \|}}

\newcommand{\inner}[3]{\ensuremath{\langle #1,#2\rangle}_{#3}}
\newcommand{\Biginner}[3]{\ensuremath{\Big\langle #1,#2\Big\rangle}_{#3}}
\newcommand{\Bigginner}[3]{\ensuremath{\Bigg\langle #1,#2\Bigg\rangle}_{#3}}

\makeatletter
\newcommand{\vast}{\bBigg@{4}}
\newcommand{\Vast}{\bBigg@{5}}
\newcommand{\vastinner}[3]{\ensuremath{\vast\langle #1,#2\vast\rangle}_{#3}}
\newcommand{\Vastinner}[3]{\ensuremath{\Vast\langle #1,#2\Vast\rangle}_{#3}}

\newcommand{\define}{\ensuremath{\triangleq}}

%--------------------------------------------
%-------Signal Spaces------------------------
%--------------------------------------------

\newcommand{\Fourier}{\ensuremath{\mathscr{F}}}
\newcommand{\InvFourier}{\ensuremath{\mathscr{F}^{-1}}}
\newcommand{\Laplace}{\ensuremath{\Lambda}}
\newcommand{\Laplacecausal}{\ensuremath{\Lambda^+}}
\newcommand{\Laplaceacausal}{\ensuremath{\Lambda^-}}

\newcommand{\Mult}[1]{\ensuremath{\mathsf{M}_{#1}}}
\newcommand{\Conv}[1]{\ensuremath{\mathsf{Conv}_{#1}}}

\newcommand{\ContrX}[1]{\ensuremath{\mathscr{C}_{r}({\real};#1)}}
\newcommand{\Contr}[1]{\ensuremath{\mathscr{C}_{r}^{#1}({\real})}}
\newcommand{\ContR}[2]{\ensuremath{\mathscr{C}_{#1}^{#2}({\real})}}
\newcommand{\ContC}[2]{\ensuremath{\mathscr{C}_{#1}^{#2}({\j\real})}}

\newcommand{\Tdist}{\ensuremath{\mathsf{T}}}
\newcommand{\Sch}{\ensuremath{\mathscr{S}(\real)}}
\newcommand{\Schcausal}{\ensuremath{\mathscr{S}[0,\infty)}}
\newcommand{\Schacausal}{\ensuremath{\mathscr{S}(-\infty,0]}}
\newcommand{\Schprime}{\ensuremath{\mathscr{S}^{\prime}(\real)}}
\newcommand{\Schprimecausal}{\ensuremath{\mathscr{S}^{\prime}[0,\infty)}}
\newcommand{\Schprimeacausal}{\ensuremath{\mathscr{S}^{\prime}(-\infty,0]}}

\newcommand{\SchprimeC}{\ensuremath{\mathscr{S}^{\prime}(\j\real)}}
\newcommand{\SchC}{\ensuremath{\mathscr{S}(\j\real)}}

\newcommand{\Contrcausal}[1]{\ensuremath{\mathscr{C}_{r}^{#1}[0,\infty)}}
\newcommand{\Contcausal}[2]{\ensuremath{\mathscr{C}_{#1}^{#2}[0,\infty)}}


\newcommand{\myL}{\mathcal{L}}

\newcommand{\Lone}{\ensuremath{\myL_{1}}}
\newcommand{\LoneR}[1]{\ensuremath{\myL_{1}^{#1}(\real)}}
\newcommand{\Lonecausal}[1]{\ensuremath{\myL_{1}^{#1}[0,\infty)}}
\newcommand{\Loneacausal}[1]{\ensuremath{\myL_{1}^{#1}(-\infty,0]}}

\newcommand{\Lonee}{\ensuremath{\myL_{1\mathrm{e}}}}
\newcommand{\LoneeR}[1]{\ensuremath{\myL_{1\mathrm{e}}^{#1}(\real)}}
\newcommand{\Loneecausal}[1]{\ensuremath{\myL_{1\mathrm{e}}^{#1}[0,\infty)}}
\newcommand{\Loneeacausal}[1]{\ensuremath{\myL_{1\mathrm{e}}^{#1}(-\infty,0]}}

\newcommand{\elltwo}[1]{\ensuremath{\ell_{2}^{#1}(\mathbb{Z}_{\geq 0})}}
\newcommand{\elltwoe}[1]{\ensuremath{\ell_{2e}^{#1}(\mathbb{Z}_{\geq 0})}}
\newcommand{\hatellinf}[1]{\ensuremath{\hat{\ell}_{\infty}^{#1}(\mathbb{T})}}

\newcommand{\Sig}[1]{\ensuremath{\mathsf{Sig}^{#1}(\real)}}
\newcommand{\SigC}[1]{\ensuremath{\mathsf{Sig}^{#1}(\j\real)}}
\newcommand{\Sigcausal}[1]{\ensuremath{\mathsf{Sig}^{#1}[0,\infty)}}
\newcommand{\Sigacausal}[1]{\ensuremath{\mathsf{Sig}^{#1}(-\infty,0]}}

\newcommand{\Ltwo}{\ensuremath{\myL_{2}}}
\newcommand{\LtwoR}[1]{\ensuremath{\myL_{2}^{#1}(\real)}}
\newcommand{\Ltwocausal}[1]{\ensuremath{\myL_{2}^{#1}[0,\infty)}}
\newcommand{\Ltwoacausal}[1]{\ensuremath{\myL_{2}^{#1}(-\infty,0]}}
\newcommand{\Ltwotaucausal}[1]{\ensuremath{\myL_{2}^{#1}[\tau,\infty)}}
\newcommand{\Ltwotauacausal}[1]{\ensuremath{\myL_{2}^{#1}(-\infty,\tau]}}
\newcommand{\LtwoTcausal}[1]{\ensuremath{\myL_{2}^{#1}[T,\infty)}}
\newcommand{\LtwoTacausal}[1]{\ensuremath{\myL_{2}^{#1}(-\infty,T]}}


\newcommand{\Ltwoe}{\ensuremath{\myL_{2\mathrm{e}}}}
\newcommand{\LtwoeR}[1]{\ensuremath{\myL_{2\mathrm{e}}^{#1}(\real)}}
\newcommand{\Ltwoecausal}[1]{\ensuremath{\myL_{2\mathrm{e}}^{#1}[0,\infty)}}
\newcommand{\Ltwoeacausal}[1]{\ensuremath{\myL_{2\mathrm{e}}^{#1}(-\infty,0]}}
\newcommand{\Ltwoetaucausal}[1]{\ensuremath{\myL_{2\mathrm{e}}^{#1}[\tau,\infty)}}
\newcommand{\Ltwoetauacausal}[1]{\ensuremath{\myL_{2\mathrm{e}}^{#1}(-\infty,\tau]}}
\newcommand{\LtwoeTcausal}[1]{\ensuremath{\myL_{2\mathrm{e}}^{#1}[T,\infty)}}
\newcommand{\LtwoeTacausal}[1]{\ensuremath{\myL_{2\mathrm{e}}^{#1}(-\infty,T]}}

\newcommand{\Linf}{\ensuremath{\myL_{\infty}}}
\newcommand{\LinfR}[1]{\ensuremath{\myL_{\infty}^{#1}(\real)}}
\newcommand{\Linfcausal}[1]{\ensuremath{\myL_{\infty}^{#1}[0,\infty)}}
\newcommand{\Linfacausal}[1]{\ensuremath{\myL_{\infty}^{#1}(-\infty,0]}}

\newcommand{\Linfe}{\ensuremath{\myL_{\infty\mathrm{e}}}}
\newcommand{\LinfeR}[1]{\ensuremath{\myL_{\infty\mathrm{e}}^{#1}(\real)}}
\newcommand{\Linfecausal}[1]{\ensuremath{\myL_{\infty\mathrm{e}}^{#1}[0,\infty)}}
\newcommand{\Linfeacausal}[1]{\ensuremath{\myL_{\infty\mathrm{E}}^{#1}(-\infty,0]}}

\newcommand{\Lp}{\ensuremath{\myL_{\rm p}}}
\newcommand{\LpR}[1]{\ensuremath{\myL_{\rm p}^{#1}(\real)}}
\newcommand{\Lpcausal}[1]{\ensuremath{\myL_{\rm p}^{#1}[0,\infty)}}
\newcommand{\Lpacausal}[1]{\ensuremath{\myL_{\rm p}^{#1}(-\infty,0]}}
\newcommand{\Lptaucausal}[1]{\ensuremath{\myL_{\rm p}^{#1}[\tau,\infty)}}
\newcommand{\Lptauacausal}[1]{\ensuremath{\myL_{\rm p}^{#1}(-\infty,\tau]}}


\newcommand{\Lpe}{\ensuremath{\myL_{\mathrm{pe}}}}
\newcommand{\LpeR}[1]{\ensuremath{\myL_{\mathrm{pe}}^{#1}(\real)}}
\newcommand{\Lpecausal}[1]{\ensuremath{\myL_{\mathrm{pe}}^{#1}[0,\infty)}}
\newcommand{\Lpeacausal}[1]{\ensuremath{\myL_{\mathrm{pe}}^{#1}(-\infty,0]}}
\newcommand{\Lpetaucausal}[1]{\ensuremath{\myL_{\mathrm{pe}}^{#1}[\tau,\infty)}}
\newcommand{\Lpetauacausal}[1]{\ensuremath{\myL_{\mathrm{pe}}^{#1}(-\infty,\tau]}}

\newcommand{\Lq}{\ensuremath{\myL_{\rm q}}}
\newcommand{\LqR}[1]{\ensuremath{\myL_{\rm q}^{#1}(\real)}}
\newcommand{\Lqcausal}[1]{\ensuremath{\myL_{\rm q}^{#1}[0,\infty)}}
\newcommand{\Lqacausal}[1]{\ensuremath{\myL_{\rm q}^{#1}(-\infty,0]}}

\newcommand{\Lqe}{\ensuremath{\myL_{\rm qe}}}
\newcommand{\LqeR}[1]{\ensuremath{\myL_{\rm qe}^{#1}(\real)}}
\newcommand{\Lqecausal}[1]{\ensuremath{\myL_{\rm qe}^{#1}[0,\infty)}}
\newcommand{\Lqeacausal}[1]{\ensuremath{\myL_{\rm qe}^{#1}(-\infty,0]}}

\newcommand{\Lr}{\ensuremath{\myL_{\rm r}}}
\newcommand{\LrR}[1]{\ensuremath{\myL_{\rm r}^{#1}(\real)}}
\newcommand{\Lrcausal}[1]{\ensuremath{\myL_{\rm r}^{#1}[0,\infty)}}
\newcommand{\Lracausal}[1]{\ensuremath{\myL_{\rm r}^{#1}(-\infty,0]}}

\newcommand{\Lre}{\ensuremath{\myL_{\rm re}}}
\newcommand{\LreR}[1]{\ensuremath{\myL_{\rm re}^{#1}(\real)}}
\newcommand{\Lrecausal}[1]{\ensuremath{\myL_{\rm re}^{#1}[0,\infty)}}
\newcommand{\Lreacausal}[1]{\ensuremath{\myL_{\rm re}^{#1}(-\infty,0]}}

\newcommand{\hatLp}{\ensuremath{\hat{\myL}_{\rm p}}}
\newcommand{\hatLpC}[1]{\ensuremath{\hat{\myL}_{\rm p}^{#1}(\j\real)}}

\newcommand{\hatLq}{\ensuremath{\hat{\myL}_{\rm q}}}
\newcommand{\hatLqC}[1]{\ensuremath{\hat{\myL}_{\rm q}^{#1}(\j\real)}}

\newcommand{\hatLone}{\ensuremath{\hat{\myL}_{1}}}
\newcommand{\hatLoneC}[1]{\ensuremath{\hat{\myL}_{1}^{#1}(\j\real)}}

\newcommand{\hatLtwo}{\ensuremath{\hat{\myL}_{2}}}
\newcommand{\hatLtwoC}[1]{\ensuremath{\hat{\myL}_{2}^{#1}(\j\real)}}

\newcommand{\hatLinf}{\ensuremath{\hat{\myL}_{\infty}}}
\newcommand{\hatLinfC}[1]{\ensuremath{\hat{\myL}_{\infty}^{#1}(\j\real)}}

\newcommand{\trunc}[1]{\ensuremath{\mathcal{T}_{#1}}}
\newcommand{\projacausal}[1]{\ensuremath{\mathcal{P}_{(-\infty,#1]}}}
\newcommand{\projcausal}[1]{\ensuremath{\mathcal{P}_{[#1,\infty)}}}
\newcommand{\PT}{\ensuremath{\mathcal{P}_{T}}}
\newcommand{\Ptau}{\ensuremath{\mathcal{P}_{\tau}}}
\newcommand{\shift}[1]{\ensuremath{\mathcal{S}_{#1}}}

\newcommand{\Hinf}{\ensuremath{\mathcal{H}_{\infty}}}
\newcommand{\HinfC}[1]{\ensuremath{\mathcal{H}_{\infty}^{#1}(\j\real)}}
\newcommand{\Htwo}{\ensuremath{\mathcal{H}_{2}}}
\newcommand{\HtwoC}[1]{\ensuremath{\mathcal{H}_{2}^{#1}(\j\real)}}

\newcommand{\Rat}{\ensuremath{\mathcal{R}}}
\newcommand{\RHinf}{\ensuremath{\mathcal{RH}_{\infty}}}
\newcommand{\RHinfC}[1]{\ensuremath{\mathcal{RH}_{\infty}^{#1}(\j\real)}}
\newcommand{\RHtwo}{\ensuremath{\mathcal{RH}_{2}}}
\newcommand{\RHtwoC}[1]{\ensuremath{\mathcal{RH}_{2}^{#1}(\j\real)}}
\newcommand{\RhatLtwoC}[1]{\ensuremath{\mathcal{R}\hat{\myL}_{2}^{#1}(\j\real)}}


\newcommand{\forallt}{\ensuremath{\text{for all}\,\,\,t \geq 0}}
\newcommand{\step}{\ensuremath{\mathsf{1}}}

\newcommand{\Test}{\ensuremath{\mathscr{D}}}
\newcommand{\pv}[1]{\ensuremath{\mathsf{pv}\left(\frac{1}{#1}\right)}}

%--------------------------------------------
%-------Robust Control Notation--------------
%--------------------------------------------

\newcommand{\rmodel}[4]{
            \left[
            \begin{array}{c|c}
                {#1} & {#2}\\
                \hline
                {#3} & {#4}
            \end{array}
            \right]
}

\newcommand{\IQC}{\mathsf{IQC}}
\newcommand{\SIQC}{\mathsf{SIQC}}
\newcommand{\HIQC}{\mathsf{HIQC}}

\newcommand{\hatPi}{\hat{\Pi}}
\newcommand{\hatPsi}{\hat{\Psi}}

\newcommand{\sector}{\mathtt{sector}}
\newcommand{\slope}{\mathtt{slope}}
\newcommand{\sat}{\mathsf{sat}}

\newcommand{\matlab}{\texttt{MATLAB}\,\,}

\newcommand{\CallierR}[1]{\mathscr{A}_{#1}(\real)}
\newcommand{\Calliercausal}[1]{\mathscr{A}_{#1}[0,\infty)}
\newcommand{\Callieracausal}[1]{\mathscr{A}_{#1}(-\infty,0]}
\newcommand{\hatCallier}[1]{\hat{\mathscr{A}}_{#1}}


\newcommand{\Clarke}{\partial_{\mathsf{C}}}
\newcommand{\VI}[2]{\mathrm{VI}(#1,#2)}
\newcommand{\prox}{\mathrm{prox}}







